Importance Weighted Actor-Critic for Optimal Conservative Offline Reinforcement Learning

We propose A-Crab (Actor-Critic Regularized by Average Bellman error), a new practical algorithm for offline reinforcement learning (RL) in complex environments with insufficient data coverage. Our algorithm combines the marginalized importance sampling framework with the actor-critic paradigm, where the critic returns evaluations of the actor (policy) that are pessimistic relative to the offline data and have a small average (importance-weighted) Bellman error. Compared to existing methods, our algorithm simultaneously offers a number of advantages: (1) It achieves the optimal statistical rate of $1/\sqrt{N}$ -- where $N$ is the size of offline dataset -- in converging to the best policy covered in the offline dataset, even when combined with general function approximators. (2) It relies on a weaker average notion of policy coverage (compared to the $\ell_\infty$ single-policy concentrability) that exploits the structure of policy visitations. (3) It outperforms the data-collection behavior policy over a wide range of specific hyperparameters. We provide both theoretical analysis and experimental results to validate the effectiveness of our proposed algorithm.

==> relatedwork.tex <==
\section{Related Work}
\label{app:related-work}

In this section, we review additional related literature not covered in the introductions.

\subsection{Dataset Coverage Assumptions}
\label{sec:related_work_coverage_assumption}
One central challenge of offline RL is the insufficient coverage of the dataset. In RL theory, concentrability is often used to characterize dataset coverage \cite{munos2007performance, scherrer2014approximate}. For example, many earlier works require all-policy $\ell_\infty$ concentrability~\citep{scherrer2014approximate,liu2019neural,chen2019information,jiang2019value,wang2019neural,liao2020batch,zhang2020variational}. Some works even require the ratio between occupancy probability induced by polices and the dataset distribution to be bounded for every time step \citep{szepesvari2005finite, munos2007performance, antos2008learning,farahmand2010error,antos2007fitted}. The work \citet{xie2020batch} makes stronger assumptions such as requiring lower bound on conditionals $\mu(a|s)$. 




Since the all-policy concentrability assumption is strong and can often be violated in practice, recent algorithms requiring only partial data coverage assumptions are developed based on single-policy $\ell_\infty$ concentrability~\citep{rashidinejad2021bridging,zhan2022offline,rashidinejad2022optimal,chen2022offline,ozdaglar2022revisiting}. However, This could still be restrictive even if only  single-policy concentrability is required since the $\ell_\infty$ concentrability is an upper bound of density ratios over all state-action pairs.

Milder versions of $\ell_\infty$ concentrability have been studied in both all-policy concentrability framework~\citep{xie2020q,xie2020batch, feng2019kernel, uehara2020minimax} or and single-policy concentrability~\citep{uehara2021pessimistic,xie2021bellman,song2022hybrid,cheng2022adversarially}. However, these works based on milder versions of $\ell_\infty$ single-policy concentrability are either computationally intractable \citep{uehara2021pessimistic, xie2021bellman} or suffer a suboptimal statistical rate~\citep{pmlr-v162-cheng22b}. 

Our work uses $\ell_2$ concentrability version, which also appears in \citet{xie2020q}. In particular, they also use weighted average Bellman error in their algorithm. However, their algorithm requires all-policy concentrability assumptions and thus cannot deal with partial dataset coverage. To the best of our knowledge among previous works, only \citet{uehara2021pessimistic} used $\ell_2$ single-policy concentrability to characterize data coverage, but their algorithm is designed for model-based settings and are computationally intractable. Another closely related work is~\citet{uehara2020minimax}, which also uses weighted average Bellman error. However, their algorithm is in the off-policy evaluation (OPE) framework, and they use $\ell_\infty$ concentrability version to characterize dataset coverage.

\subsection{Conservative offline reinforcement learning}

To address partial dataset coverage in offline RL, 
a line of recent applied works  studies conservative algorithms, which can be divided into several categories. 

The first category enforces the learned policy to be close to the behavior policy (or equivalently, dataset), which ensures that candidate policies not well covered by the dataset are eliminated. This can be accomplished by either adding constraints explicitly~\citep{fujimoto2019off,kumar2019stabilizing,wu2019behavior,jaques2019way, siegel2020keep,ghasemipour2020emaq, fujimoto2021minimalist}, implicitly~\cite{peng2019advantage, nair2020accelerating}, or by importance sampling with bounded ratio~\citep{swaminathan2015batch, liu2019off, nachum2019algaedice,  zhang2020gradientdice, Zhang2020GenDICE:, lee2021optidice}. 

The second category consists of model-based methods such as adversarial model learning \cite{rigter2022rambo}, learning pessimistic models \cite{kidambi2020morel, guo2022model},   using model ensembles to form penalties\cite{yu2020mopo}, or combining model and values \citep{yu2021combo}.

The last category  aims to learn conservative values such as fitted Q-iteration using conservative update \citep{liu2020provably}, conservative Q-learning (CQL) \citep{kumar2020conservative}, critic regularization \citep{kostrikov2021offline}, and subtracting penalties \citep{rezaeifar2022offline}. 

On the theoretical side, many works use some form of uncertainty quantification to design to ensure pessimism~\citep{yin2021towards, kumar2021should, uehara2021representation,  yin2022near, zhang2022corruption, yan2022efficacy, shi2022distributionally, wang2022gap}. Except for uncertainty quantification, in linear function approximation settings, \citet{zanette2021provable} uses value function perturbation combined with the actor-critic method. Recent advances in the theory of pessimistic algorithms include MIS \cite{zhan2022offline, chen2022offline} and adversarially trained actor-critic (ATAC) \cite{pmlr-v162-cheng22b}. In particular, our algorithm is built based on MIS combined with the actor-critic method.
